Investigations into the impact of astronomical phenomena on the terrestrial biosphere and climate

This thesis assesses the influence of astronomical phenomena on the Earth's biosphere and climate. I examine in particular the relevance of both the path of the Sun through the Galaxy and the evolution of the Earth's orbital parameters in modulating non-terrestrial mechanisms. I build models to predict the extinction rate of species, the temporal variation of the impact cratering rate and ice sheet deglaciations, and then compare these models with other models within a Bayesian framework. I find that the temporal distribution of mass extinction events over the past 550 Myr can be explained just as well by a uniform random distribution as by other models, such as variations in the stellar density local to the Sun arising from the Sun's orbit. Given the uncertainties in the Galaxy model and the Sun's current phase space coordinates, as well as the errors in the geological data, it is not possible to draw a clear connection between terrestrial extinction and the solar motion. In a separate study, I find that the solar motion, which modulates the Galactic tidal forces imposed on Oort cloud comets, does not significantly influence this cratering rate. My dynamical models, together with the solar apex motion, can explain the anisotropic perihelia of long period comets without needing to invoke the existence of a Jupiter-mass solar companion. Finally, I find that variations in the Earth's obliquity play a dominant role in triggering terrestrial deglaciations over the past 2 Myr. The precession of the equinoxes, in contrast, only becomes important in pacing large deglaciations after the transition from the 100-kyr dominant periodicity in the ice coverage to a 41-kyr dominant periodicity, which occurred 0.7 Myr ago.

==> biodiversity_bkp.tex <==
\section{Chapter Summary}\label{abstract_biodiversity}

The terrestrial fossil record reveals a significant variation in the extinction and origination rates of species over the past half billion years. Numerous studies have claimed an association between this variation and the motion of the Sun around the Galaxy, invoking cosmic rays, gamma rays and comet impacts modulated by this motion as the cause of biodiversity variation. However, some of these studies have suffered from methodological problems or have been based on coarse assumptions (such as a strict periodicity of the solar orbit).  Here we investigate this link in more detail, using a model of the Galaxy to reconstruct the solar orbit, from which we derive a predictive model of the variation of the extinction rate due to astronomical mechanisms.  We compare these predictions with several paleontological data sets, and compare this predictive power -- or evidence -- with that of numerous non-orbital reference models.  Our approach involves Bayesian model comparison, which takes into account the uncertainties in the paleontological data as well as the distribution of solar orbits consistent with the uncertainties in the astronomical data.  We find that, for all data sets, various versions of the orbital model are not favored beyond simpler analytic models.  In particular, the time distribution of mass extinction events can be just as well explained as a uniform random distribution as with any other of the models tested. We also find that the continuous variation of the extinction rate constructed by Rohde \& Muller (as well as another from Alroy et al.) does not show significant evidence for periodicity, in contrast to claims made elsewhere. Simpler models will do.  Although our negative results on the orbital model are reasonably robust to changes in the Galaxy model, the Sun's coordinates and the errors in the data, this does not rule out a relevance of astronomical mechanism per se.  However, it does seem that with the current data it would be difficult to draw a positive conclusion on there being a general connection between solar motion and biodiversity variations on the Earth.

\section{Introduction}\label{sec:introduction_biodiversity}

\subsection{Background}

During the course of the Earth's history, evolution has produced a wide and constantly changing variety of life. This is particularly apparent from about 550\,Myr ago -- the start of the Phanerozoic eon -- when hard-shelled animals first appeared and were preserved in the fossil record. Since then we observe an overall increase in the diversity of life, but with significant variation \citep{sepkoski02, rohde05, alroy08sci}. The largest and most rapid decreases in biodiversity -- defined here are the number of genus extant at any one time -- are referred to as mass extinctions.

The cause of these variations in biodiversity in general, and mass extinctions
in particular, have been the subject of intense study and speculation for over
a century. (This has often focused on the marine fossil record because fossil
preservation is more likely in a marine environment.)  Many mechanisms have
been proposed for the observed variation, which we can place into four groups.

%%% More/better references here, 
%%%%%I have cancel "and perhaps most obviously"
%%%%%because there is a counterpart for the red queen hypothesis: Court Jester
%%%%%Hypothesis.  
First, the variations are the result of inter-species interactions. Species
compete for limited resources, and as one species evolves to compete in this
struggle for survival, so other species will evolve too.  This paradigm is
also known as the ``Red Queen'' hypothesis \citep{van-valen73,
  benton09}.  And recent ecological study indicates that the nested
interaction between species can minimize competition and enhance biodiversity
\citep{sugihara09}.  However, these biotic factors may not be the major cause of
large patterns of biodiversity \citep{benton09, alroy08}.
% \citep{alroy08,alroy10}
%Such population dynamics generally include both biotic and abiotic factors,
%the later
%reflecting the fact that over geological time scales the environment is constantly changing \citep{peters05,heim11,ipcc}. 

Second, the environment changes with time, and species will evolve in response
to this.  This is also known as the ``Court Jester'' hypothesis
\citep{barnosky01,benton09}.  Some of these geological changes are relatively
slow -- such as plate tectonics, atmospheric composition, changes of global
climate \citep{sigurdsson88, crowley88, wignall01, marti05, feulner09,
  wignall09}. But others may be more rapid or dramatic. Large-scale volcanism,
for example, would inject dust, sulfate aerosols and carbon dioxide into the
stratosphere, which could cause a short-term global cooling, reduce
photosynthesis, generate long periods of acid rain and ultimately produce
long-term global warming (about $10^5$ years) \citep{marti05}.

Third, extraterrestrial mechanisms could be involved, either through a direct
impact on life or by changing terrestrial climate. The tilt of the Earth's
axis is responsible for the seasons, and variations in the Earth's orbit
(mostly its eccentricity) over ten to one hundred thousand year time scales
are responsible for the ice ages \citep{hays76, muller00}. Mechanisms on longer
time scales are also likely to play a role. These include solar variability
\citep{shaviv03,lockwood05,lockwood07}, asteroid or comet impacts
\citep{shoemaker83,alvarez80,glen94}, cosmic rays \citep{shaviv05, sloan08}, supernovae (SNe) and gamma-ray burst \citep{ellis95,melott08} (for a review see
\cite{bailer-jones09}). For example, cosmic rays could influence the Earth's
climate if they play a significant role in cloud formation (through the
formation of cloud condensation nuclei) \citep{carslaw02,kirkby08}.
%%% Add REFS:Carslaw et al. 2002, Kirkby 2007
Secondary muons resulting from cosmic rays -- as well as high energy gamma rays
from SNe -- could kill organisms directly or damage their DNA
\citep{thorsett95, scalo02, atri12}.

Finally, the apparent variation may be, in part, the result of uneven preservation and sampling bias \citep{raup72, alroy96, peters05}. Fossilization is relatively rare and some animals are more likely to be preserved than others.  Furthermore, the degree of marine preservation depends on the amount of continental outcrop available at any time, and this depends on the sea level \citep{hallam89, holland12}.  The number of species or genera living at any one time is not observed but must be reconstructed from the times at which species appear and disappear, which implies some kind of sampling or modeling. This can introduce a bias, although it may be diminished to some degree by various techniques \citep{alroy01, alroy10}.

These four types of cause are of course not mutually exclusive. They are all likely to have played a role at some point, and furthermore will have interacted. For example, an asteroid impact could release so much carbon dioxide that long-term global warming has the biggest impact on biodiversity. Alternatively, a cool period would lower sea levels, leaving less continental shelf for the preservation of marine fossils, even though biodiversity itself may be unchanged.

Given the limited geological record, untangling the relevance of these different causes in most individual cases is difficult, if not impossible. More promising, however, might be an attempt to identify the overall, long-term significance of these potential causes. The goal of this article is to do that for extraterrestrial phenomena. 

%%% REFS: fit in these/others as appropriate.
% \citep{bahcall85,gies05,melott10, melott12}
% \citep{shaviv02, sanchez01} 
% \citep{raup84,rohde05}. 
Many of the astronomical mechanisms mentioned above are ultimately caused by
the presence of nearby stars. Stars turn supernovae, the source of gamma rays,
and their remnants are a major source of cosmic rays \citep{koyama95}. Stars
perturb the Oort cloud, the main source of comets in the inner solar system
\citep{rampino84,sanchez01}. Broadly speaking, when the Sun is in a
region of higher stellar density, it is more exposed to extraterrestrial
mechanisms of biodiversity change. In its orbit around the Galaxy (once every
200--250\,Myr or so), the Sun's environment changes. In particularly, it
oscillates about the Galactic plane with a (quasi) period of 50--75\,Myr
\citep{bahcall85}, and in doing so moves through regions of more intense star
formation activity in the Galactic plane. This is particularly true if the Sun
crosses spiral arms \citep{gies05, leitch98}, which it may do every 100-200\,Myr or so.  

Such changes in the solar environment have been used as the basis for many
claims of a causal connection between the solar motion and mass extinctions
and/or climate change on the Earth. Typically, authors have identified a
periodicity in the fossil record and then connected this to a plausible
periodicity in the solar motion \citep{alvarez84, raup84, davis84, muller88,
  shaviv03, rohde05, melott10, melott12}. These comparisons are fraught with
problems, however, some of which remained unmentioned by the authors. The
first is the fact that the solar motion and past environment is poorly
constrained by the astronomical data, so a wide range of
plausible periods are permissible \citep{overholt09, mishurov11}, yet the
coincident one is naturally chosen. Second comes the fact that the solar
motion is not strictly periodic even under the best assumptions. Third, many
of these studies have not performed a careful model comparison. Typically they
identify the best fitting period assuming the periodic model to be true, but
fail to accept that a non-periodic model might explain the data \citep{kitchell84, stigler87}. In some cases a significance test is introduced to exclude a specific noise model, but these are often misinterpreted and the resulting significance overestimated.  The reader is referred to \cite{bailer-jones09} for an in-depth review and references.

%%% Maybe we can fit some of this or these references in.
% However, many researchers pointed out that the methods used in the above studies are problematic. One problem is that some studies only fit their models to the data rather than infer their models from the data. For an instance, Gies and Helsel tried to find a connection between the Sun's spiral arm crossings with the ice ages or mass extinction events in the last 500 Myr \citep{gies05}. They have oversimplified the integration of the Sun's motion by taking a fixed initial conditions of the Sun. In addition, they have assumed a connection between ice ages and spiral arm crossings, then they adjusted the pattern speed of the spiral arm to fit the occurrence time of crossings to the ice ages. This method is called model fitting rather than model inference. Another common problem is the statistics used to find the periodicity in the biodiversity or mass extinction data. These studies always use maximum likelihood or periodogram to find the favored period and claim that the biodiversity data follow the periodic pattern \citep{raup84, raup86, rohde05, lieberman09}. However, the periodicity could be artificial without using robust model inference method \citep{kitchell84,stigler87,bailer-jones09,bailer-jones11}.

\subsection{Overview}\label{sec:overview_biodiversity}

Here we attempt a more systematic assessment of the possible role of the solar orbit in modulating extraterrestrial extinction mechanisms. Our approach is new in a number of respects, because we: (1) do a numerical reconstruction of the solar orbit (rather than just assuming it to be periodic); (2) take into account the observational uncertainties in that reconstruction; (3) use models which predict the variation of probability of extinction with time (rather than assuming that extinction events occur deterministically, for instance); (4) do proper model comparison (rather than using p-values in a contrived significance test); (5) compare not only the orbital model with the fossil record but also numerous reference (non-orbital) models, such as periodic, quasi-periodic, trend, periodic with constant background, etc.

%%%%%% Rene has some comments for this: he think the mass extinction may not
%%%%%% be linearly related to the stellar density which might compromise our
%%%%%% results. Do we need to take this into account or give the model of mass
%%%%%% extinction response to the extraterrestrial causes?
Our method is as follows. Adopting a model the distribution of mass in the
Galaxy, we reconstruct the solar orbit over the past 550\,Myr by integrating
the Sun's trajectory back in time from the current phase space coordinates (position and velocity). This gives us a time series of how the stellar density in the vicinity of the Sun has varied over the Phanerozoic. We then assume that this density is approximately proportional to the terrestrial extinction probability (per unit time). That is, we adopt a non-specific kill mechanism linking the solar motion to terrestrial biodiveristy.  This is naturally a strong and rather simple assumption, but it should be emphasized that we are interested in the overall plausibility of extraterrestrial phenomena rather than trying to identify a specific cause of individual extinction events. The resulting time series is then compared to several different reconstructions of the biodiversity record.

A significant source of uncertainty in the reconstructed solar orbit are the
current phase space coordinates (or ``initial'' conditions). We therefore
sample over these to build up a set of (thousands of) possible solar orbits,
and compare each of these with the data. The comparison is done by calculating
the likelihood of the data for each orbit. Rather than finding the single most
likely orbit, we calculate the average likelihood over all orbits. This is
important, because it properly takes into account the uncertainties (whereas
selecting the single most likely orbit would ignore them entirely). Indeed,
these initial conditions can be considered as the six parameters of this
orbital model (for a fixed Galactic mass distribution). We are, therefore,
averaging the likelihood for this model over the prior plausibility of each of
its parameters. This average -- or marginal -- likelihood is often called the
``evidence''.  This is just the standard, Bayesian approach to model
assessment, which avoids the numerous flaws of hypothesis testing
\citep{jeffreys61, winkler72, mackay03}, but unfortunately it has seen little
use in this field of research.
%%%%%Rene has asked whether the last sentence is necessary. 

The next step is to compare this evidence with that calculated for various reference models (sometimes called ``noise'' or ``background'' models, depending on the context). One such model is a pure periodic model, parameterized by an amplitude, period and phase. Here we also generate a large number of realizations of the model for different combinations of the parameters, calculate the likelihood of the data for each, and average the results. This averaging also plays the crucial role of accommodating the complexity of the model. A complex model with lots of parameters can normally be made to fit an arbitrary data set well. That is, it will give a high maximum likelihood.  But that does not make it a good model, precisely because we know that it could have been made to fit any data set well! Such models are highly tuned, so while the maximum likelihood fit may be very good, a small perturbation of the parameters results in poor predictions. Unless well-supported by the data, such models are less plausible. A simpler model, in contrast, may not give such an optimal fit, but it is normally more robust to small perturbations of the model parameters or the data, so gives good fit over a wider portion of the parameter space. The model evidence embodies and quantifies this trade-off, which is why it -- rather than the maximum likelihood -- should be used to compare models.

We have selected four different data sets for our study. The first two are compilations of the variation of extinction rate over time, from \cite{rohde05} and \cite{alroy08sci}. In the latter we use the extinction rate standardized to remove the sampling bias. Both report a magnitude as a function of time.
The second two data sets just record the time of mass extinction events. Here we take the times of the ``big 5'' mass extinctions and 18 mass extinctions identified by \cite{bambach06} based on Sepkoski's earlier work \citep{sepkoski86}.  Each mass extinction is represented as a (normalized) Gaussian on the time axis, the mean representing the best estimate of the date of the event and the standard deviation the uncertainty. We refer to these as ``discrete'' data sets, as they just list the discrete dates at which events occur (we do not use any magnitude information). The two rate data sets we therefore refer to as ``continuous'' (even though in practice the rates are also recorded at discrete time points).

The paper is arranged as follows. We first introduce the data sets. In Section~\ref{sec:bayes} we build time series models to predict the extinction rate over the past 550\,Myr. In Section~\ref{sec:solarorbit_biodiversity} we describe how we reconstructed the solar orbit, and also quantify the degree of periodicity typically present (as a strict periodicity has often been assumed in the past).  In Section~\ref{sec:result_biodiversity} we calculate and compare the evidences for the various models and data sets and test the sensitivity of the results to the model parameters and uncertainties in the data.  We conclude in Section~\ref{sec:conclusion_biodiversity}.

\section{\label{sec:paleontological_biodiversity} Paleontological data}

We adopt four data sets: two discrete time series (sequence of time points
with age uncertainties) giving the dates of mass extinctions, and two
continuous time series giving the smoothed and normalized extinction rate as a
function of time.

\subsection{\label{sec:datadiscrete_biodiversity} Discrete data sets}

Sepkoski and others have identified five extinction events to be ``mass
extinctions'' \citep{sepkoski86}, often referred to as the ``big
five''. However, other studies have identified different candidates for these,
or have identified a ``big $N$'' for some other value of $N$. For example,
Bambach et al.\ identify three mass extinction events as being globally
distinct \citep{bambach04}.  Here we adopt a set of 18 mass extinction events
(or B18) selected by \cite{bambach06} using an updated Sepkoski genus-level database. They are consistently identifiable in different biodiversity data sets and when using different tabulation methods. The second of our discrete data sets is the ``big five'' as identified from amongst the B18. Other choices of events are of course possible and our results will, in general, depend on this choice (although as we'll see the results are rather consistent).

The times and durations of the events are listed in
Table~\ref{tab:ext-b5-b18}.  The time, $\tau$, is the mid-point between the
start age and end age of the substage in which the extinction occurred, and
the duration, $d$, is the difference between these.  Assuming the extinction
to have taken place more rapidly than this difference, then $\tau$ is our
(best) estimate of the true (but unknown) time, $t$, at which the extinction
occurred, and $d$ is proportional to our uncertainty.  Uncertainty is
represented by probability, so we can interpret an ``event'' as the
probability distribution $P(\tau | t, d)$: this is the probability that we would measure the event time as $\tau$, given $t$ and $d$.  We might want to represent this as a rectangular (``top-hat'') distribution of mean $t$ and width $d$, but this assigns exactly zero probability outside the substage duration, which assigns too much certainty to the start and end ages. So we instead consider each event as a Gaussian distribution with mean $t$, and standard deviation $\sigma$ equal to the standard deviation of the rectangular distribution, which is $\sigma = d/\sqrt{12}$.  Note that the intensity of the mass extinction is not taken into account. A Gaussian is normalized, so its peak value is determined by its standard deviation (Fig.~\ref{fig:data}).\footnote{One might think that a more natural interpretation of an event is $P(t | \tau, d)$, the probability that the true event occurs at $t$ given the measurements. That would also be possible, but here we are considering the measurement model (or noise model), i.e.\ given some true time of the event, what possible times might we measure, the discrepancy arising on account of the finite precision of our measurement process.}

\begin{table}
\caption{The B18 mass extinction events, with the B5 shown in bold. BP = before present.}
\centering
\begin{tabular}{l c}
\hline
\hline
       Time ($\tau$) / Myr BP & Substage duration ($d$) / Myr\\
\hline
3.565&3.53\\
35.550&3.30\\
{\bf 66.775}&{\bf 2.55}\\
94.515&2.03\\
146.825&2.65\\
182.800&7.00\\
{\bf 203.750}&{\bf 8.30}\\ 
{\bf 252.400}&{\bf 2.80}\\
262.950&5.10\\
324.325&4.15\\
361.600&4.80\\
{\bf 376.300}&{\bf 3.60}\\
386.925&3.25\\
{\bf 445.465}&{\bf 3.53}\\
489.350&2.10\\
495.725&2.15\\
499.950&2.10\\
519.875&2.75\\
\hline 
\end{tabular}
\label{tab:ext-b5-b18}
\end{table}
%%%%% I have changed the caption a little, "these can be interpreted as the
%%%%% extinction probability density function, which is ... to the extinction
%%%%% proportion per unit time." 
\begin{figure*}
\centering
\includegraphics[scale=0.7]{Extinction_data_plot.eps}
\caption{The four data sets used in this study. The top row shows the discrete
  data sets: the B5 (left) and B18 (right) mass extinction events. These can
  be interpreted as the extinction probability density function(PDF), which is proportional to the extinction proportion per unit time.
The bottom row shows the continuous data sets, which give the extinction rate per unit time:
RM (left) and A08 (right).}
\label{fig:data} 
\end{figure*} 

\subsection{\label{sec:continuous_biodiversity} Continuous data sets}

%%% Note that I have changed your notation. Extinction rate is now E(t), not R(t), to avoid confusion later with R
%%% being the cylindrical radial coordinate
The discrete data sets are naturally biased in that they only select periods of high extinction rate. It may well be that extraterrestrial phenomena are only relevant in causing (or contributing to) mass extinctions, but a priori it is natural to ask how well the overall extinction rate variation can be predicted by the orbital and reference models.  The extinction rate is the fraction of genera which go extinct in a stratigraphic substage divided by its duration, and we denote it $E(t)$. This is directly proportional to the variation of extinction probability per unit time.
%This absolute value of this could be overestimated if the extinction recorded in fact took place over a shorter period shorter than the temporal resolution of the substage, but this still provides a useful indicator of change in extinction  \citep{bambach06}.
%%% - not really!
For one of our extinction rate data sets we use the linearized and
interpolated data set constructed by \cite{rohde05} as
reported in \cite{bambach06}. We denote this RM. The other data set
we use is the ``three-timer'' extinction rate from the
Paleobiology database\footnote{paleodb.org} \citep{alroy08sci}. The data are
binned into 48 intervals, averaging 11.0 Myr in duration. The counts are
derived from 281,491 occurrences of 18,541 genera within 42,627 fossil
collections. We use the data set processed using their subsampling method to
reduce the sampling bias, and denote this A08. 
%%% Be more specifc here, as I think they report several data sets
Both data sets are reported as lists of extinction rates at specific times,
$\{r_j, \tau_j\}$. These two continuous data sets are plotted in the lower row of Fig.~\ref{fig:data}.

\section{\label{sec:tsmodels_biodiversity} Time series models}

After defining the data sets, we build time series models to predict the extinction rate. The time series models appear in the equation for the likelihood in the form $P(t | \theta, M)$, i.e.\ the extinction probability (per unit time) as a function of time predicted by model $M$ at parameters $\theta$. It is important to realize that this probability density function (PDF) over $t$ is normalized, i.e.\ integrates over all time to unity. This is crucially important to model comparison, because a model which assigns a lot of probability to extinctions occurring at some time must necessarily assign lower probability elsewhere. This is because we are not trying to model the absolute value of the extinction rate, but just how it varies in time.

In addition to specifying the functional form of the models we must also specify the prior probability distribution of the model parameters, $P(\theta | M)$. This describes our prior knowledge of the relative
probability of different parameter settings. For example, given the time scale
in the data, we are not interested in models with time scales less than a few
million years or more than a few hundred million years. It is often difficult to be precise about priors, and the evidence and therefore Bayes' factors often depend on the choice. The choice of prior must therefore be considered part of the model (e.g.\ ``periodic model with permissible periods between 10 and 100\,Myr'' is distinct from ``periodic model with permissible periods between 50 and
60\,Myr''). We should further investigate the sensitivity of the results to
changes in the prior, something we will do later in Section~\ref{sec:sensitivity_biodiversity}. Except for the orbital model, we adopt a uniform prior over all model parameters over the range specified in Table~\ref{tab:prior}.

%%% Do you really use cosine in PNB/PB but sine in QPM?  If possible, change the definition to be cosine in both cases. That way you can have the same value of the phase, beta, in {fig:models}, although you need to check that you don't refer to the phase, beta, elsewhere in the paper.
\begin{table*}
\centering
\caption{The mathematical form of the time series models and their corresponding parameters. Time $t$ increases into the past and $P_u(t|\theta, M)$ is the unnormalized extinction probability density predicted by the model.}
\begin{tabular}{l c r}
\hline
\hline
model name&$P_u(t|\theta,M)$&parameters\\
\hline
Uniform&1&none\\
RNB/RB&$\sum_{n=1}^{N}\mathcal{N}(t; \mu_n,\sigma)$+$B$&$\sigma$, $N$, $B$\\
PNB/PB&$1/2\{\cos[2\pi(t/T+\beta)]+1\}$+$B$&$T$, $\beta$, $B$\\
QPM&$1/2\{\cos[2\pi t/T + A_Q \cos(2 \pi t/T_Q) +\beta]+1\}$&$T$, $\beta$, $A_Q$, $T_Q$\\
SP&$[1+e^{(t-t_0)/\lambda}]^{-1}$&$\lambda$, $t_0$\\
SSP&PNB+SP&$T$, $\beta$, $\lambda$, $t_0$\\
OM/SOM&$n(\overrightarrow{r_\odot}(t),\overrightarrow{v_\odot}(t))$&$\overrightarrow{r_\odot}(t=0),~\overrightarrow{v_\odot}(t=0),~h$\\
\hline
\end{tabular}
\label{tab:models}
\end{table*}

\begin{table*}
\centering
\caption{Range of parameters adopted in the model prior parameter distributions.
Except for OM/SOM, a uniform prior for all parameters for all models is adopted which is constant inside the range shown, and zero outside. The prior PDF of parameters in the OM/SOM
  model is Gaussian and specified by the uncertainties in the initial conditions.}
\begin{tabular}{l c}
\hline
\hline
model name & range of prior \\
\hline
Uniform& None\\
RNB/RB & $\sigma=10$~Myr, $N\in\{5,18\}$, $B\in[0,\frac{1}{\sqrt{2\pi}\sigma}]$\\
PNB/PB & $10<T<100$, $0<\beta<2\pi$, $B\in[0,1]$\\
QPM &$10<T<100$, $0<\beta<2\pi$, $0<A_Q<0.5$, $200<T_Q<500$\\
SP &$-100<\lambda<100$, $100<t_0<500$\\ 
SSP &$10<T<100$, $0<\beta<2\pi$, $-100<\lambda<100$, $100<t_0<500$\\ 
%%% I do not understand how TH and B are defined. See below my comment under the SOM section, then
%%% replace TH and B with h.
OM/SOM & initial conditions (see Table~\ref{tab:initialconditions}), h=0\\
\hline
\end{tabular}
\label{tab:prior}
\end{table*}


%%% See comment above to see whether you can have beta=0 for both black and blue curves.
%%% Blue and black are often hard to distinguish. I suggest you swap the colours of the blue and red lines.
\begin{figure}
\centering
\includegraphics[scale=0.7]{models_schematic.eps}
\caption{Time series models. The black line shows the PNB model with $T=$\,100\,Myr, $\beta=0$. The red line shows the QPM model with $T=$\,100\,Myr, $\beta=0$, $A_Q=0.5$ and $T_Q=$\,200\,Myr; The blue line shows the SP model with $\lambda=$\,50\,Myr and $t_0=$\,200\,Myr.}
\label{fig:models}
\end{figure}

Table~\ref{tab:models} summarizes the functional form of the models, which are now briefly described. 
Fig.~\ref{fig:models} plots examples of some of these models.
The range of the data is taken to be 0--550\,Myr BP.
\begin{description}
\item[Uniform] Constant extinction PDF over the range of the data. This has no parameters.

\item[RB/RNB] This is a form of random model in which a set of $N$ times are drawn at random from a uniform distribution extending over the range of the data. A Gaussian with standard deviation $\sigma=$\,10\,Myr is assigned to each of these, and then a constant $B$ added before normalizing. This is the RB model.  The RNB (``random no background'') model is just the special case of $B=0$, which produces a model which is similar to our discrete data. 
In practice we fix $N$ and $B$ and calculate the evidence by averaging over a large number of realizations of the model. Specifically, when modeling the B5 and B18 data sets we fix $B=0$, and $N=5,18$ respectively. 

\item[PB/PNB] This is a periodic model of period $T$ and phase $\beta$ (model PNB). There is no amplitude parameter because the model is normalized over the time span of the data. Adding a background $B$ to this simulates a periodic variation on top of a constant extinction probability (model PB).

\item[QPM] A strictly periodic model is rather rigid, whereas a model which allows small variations in the period is more plausible a priori. In the quasi-periodic model the phase becomes  a sinusoid with amplitude $A_Q$, period $T_Q$ and phase $\theta$ (it becomes the same as the PNB model if $A_Q=0$). 

\item[SP] This models a monotonically increasing or decreasing nonlinear trend in the extinction PDF using a sigmoidal function characterized by the steepness of the slope, $\lambda$ and the center of the slope, $t_0$. In the limit that $\lambda$ becomes zero the model becomes a step function at $t_0$, and in the limit of very large $\lambda$ becomes the uniform model.

\item[SSP] This combines SP and PNB.

\item[OM/SOM] This is the (semi)-orbital model, and will be defined in Section~\ref{sec:solarorbit_biodiversity}.
\end{description}


\section{\label{sec:solarorbit_biodiversity} Model of the solar orbit}

We now reconstruct the orbit of the Sun around the Galaxy over the past 550\,Myr. This is done by integrating its path back in time through a fixed gravitational potential, described in Section~\ref{sec:galaxy}. (Gravity is a conservative force, so the system can be integrated backwards as well as forwards in time.) It has often been assumed that the solar orbit is periodic with respect to crossings of the Galactic plane and/or spiral arms; we investigate this numerically in Section~\ref{sec:periodicity_biodiversity}.  The stellar mass distribution corresponding to the potential gives the local stellar density which the Sun experiences in its orbit. In Section~\ref{sec:OBM_biodiversity} we will use this to derive the variation in the expected extinction rate.

\subsection{Numerical method}\label{sec:numerical}

To calculate the motion of a body through the potential from given initial conditions, we solve Newton's equations of motion, which in cylindrical coordinates are
\begin{eqnarray}
\ddot{R} -R\dot\phi^2 &=& -\frac{\partial\Phi}{\partial R} \nonumber \\
R^2 \ddot{\phi}+2R\dot{R}\dot{\phi} &=& -\frac{\partial\Phi}{\partial\phi} \nonumber \\
\ddot{z} &=& -\frac{\partial \Phi}{\partial z} 
\end{eqnarray}
We solve these equations by numerical integration using the {\tt lsoda} method
implemented in the R package {\tt deSolve}, with a time step of 0.1\,Myr. 
%%%%% Here I have taken the advice from Anthony into account, i.e. mention
%%%%% that the analytical solution of vertical motion is possible. However, to
%%%%% make it simple, we choose to simulate the solar orbits as a whole. 
In principle, the vertical motion of the Sun can be solved analytically if we
consider a potential varying only in the z direction. Actually, the motion in
the radial direction will slightly change the potential. Thus it is necessary
to use numerical methods to solve the above equations of solar motions. 

The initial conditions are the current phase space coordinates (three spatial
and three velocity coordinates) of the Sun. These are derived from
observations with a finite accuracy, so our initial conditions are Gaussian
distributions, with mean equal to the estimated coordinate and standard
deviation equal to its uncertainty (Table~\ref{tab:initialconditions}). In
order to calculate an orbit we first draw the initial conditions at random
from these prior distributions, and a large number of draws gives us a
sampling of orbits which will be used later \footnote{As gravitational systems are non-dissipating, the dynamics are reversible.}. 

\begin{table*}
\caption{The current phase space coordinates of the Sun, represented as
  Gaussian distributions, and used as the initial conditions in our orbital
  model \citep{eisenhauer03,majaess09,dehnen98b}.}
\centering
\begin{tabular}{l*5{c}r}
\hline
\hline
     &$R$/kpc&$V_R$/kpc~Myr$^{-1}$&$\phi$/rad&$\dot\phi$/rad~Myr$^{-1}$&z/kpc&$V_z$
/kpc~Myr$^{-1}$\\
\hline
mean &8.0  &-0.01              & 0        & 0.0275
&0.026&0.00717\\
standard deviation &0.5& 0.00036&0         &0.003
&0.003&0.00038\\
\hline
\end{tabular}
\label{tab:initialconditions}
\end{table*}

%%%%% Here, I have added some sentences to citep the references for the initial
%%%%% conditions. 
The distance from the Sun to the
center of the Galaxy is given according to the astrometric and spectroscopic
observations of the stars near the black hole of the Galaxy
\citep{eisenhauer03}. The Sun's displacement from the galactic plane is
calculated from the photometric observations of classical Cepheids by
\cite{majaess09}. The velocity is calculated from Hipparcos data by \cite{dehnen98b}.

There is, of course, significant uncertainty not only in the value of the
parameters of the potential we have adopted, but also in the functional form
of our model. It is undoubtedly a gross simplification of the true potential of
the Galaxy, so specific numerical values of quantities such as orbital periods
and amplitudes inferred may not be interpreted too literally. Unfortunately it
is difficult to do much better with the current data. However, our goal is not to derive specific values, but rather to look at the extent of the variation of the solar orbit when one takes into account sources of uncertainty. Here we limit that uncertainty to the current phase space coordinates.
%%% We should come back to this point later, after the likelihood analysis. That is, once we additionally take into
%%% around the uncertainty in the potential, the evidence for the orbital model is presumably lowered even further.

\subsection{Morphology of spiral arms}\label{sec:arm_biodiversity}

According to the Eqn. \ref{eqn:phi_spiral}, the shape of the arms is shown in the left panel of Fig.~\ref{fig:spiralzorbit}. The arms rotate rigidly with constant angular velocity (or pattern speed) of $\Omega_p=20$\,km\,s$^{-1}$\,kpc$^{-1}$ \citep{martos04, drimmel00}.

\begin{figure*}
\centering
\includegraphics[scale=0.7]{arm_zorbit.eps}
\caption{The solar orbit in the Galactic plane (left) and perpendicular to the
  plane (right). The orbit in the left panel is in a reference frame rotating with the spiral arms.} 
\label{fig:spiralzorbit} 
\end{figure*}

We will only use the morphological parameters in table \ref{tab:spiralarmpar} to simulate solar orbits and test the periodicity of the simulated orbits. In Section~\ref{sec:sensitivity_biodiversity}, we will find that the gravitational perturbation of spiral arms will not significantly change the evidences for orbital models. However, we will use parameters listed in Table \ref{tab:model_par} to calculate the local stellar density in Section~\ref{sec:OBM_biodiversity}. 

\begin{table*}
\caption{The morphological and density parameters of the spiral arms. Notice
  that the parameters for stellar density are applicable to both of the two arms.}
\centering
\begin{tabular}{lcccc}
\hline
\hline
\multicolumn{5}{c}{parameters for morphology}\\\hline
arm&$\alpha$&$R_{min}$/kpc&$\phi_{min}$/rad&extent/kpc\\\hline
1        & 4.25 & 3.48 & 0.26 & 6.0\\
$1^\prime$&4.25  & 3.48 & 3.40 & 6.0\\\hline
\hline
\end{tabular}
\label{tab:spiralarmpar}
\end{table*}

\subsection{\label{sec:periodicity_biodiversity} Periodicity test}
In previous studies of the impact of astronomical phenomena on the terrestrial biosphere, it has frequently been assumed that the solar motion shows strict periodicities with respect to its motion perpendicular to the Galactic plane, and sometimes also with respect to spiral arm crossings. We investigate this here using our numerical model.

For each orbit $k$, we calculate the intervals between successive
crossings, $\{\Delta t^i\}_k$, (separately for midplane and spiral arm
crossings), where $i$ indexes the crossing. We then calculate the sample
mean and sample standard deviation of these intervals for each orbit
%%% you had the equation for SD wrong. Please ensure it was correct in your
%%% code!
%%%%% Maybe we should use N_k-2 instead, because we only select a segment of
%%%%% the whole solar motion. So the sample standard deviation is proper to be
%%%%% used here. 
\begin{eqnarray}
\overline{\Delta t_k} &=& \frac{1}{N_k-1}\sum_{i=1}^{N_k-1} \Delta t_k^i\\
\sigma_k &=& \sqrt{\frac{1}{N_k-2} \sum_{i=1}^{N_k-1} (\Delta t_k^i-\overline{\Delta t_k})^2} \ ,
\end{eqnarray}
%where $\Delta t_k^i\equiv T_k^{i+1}-T_k^i$ ($T_k^i$ is the time of the $i^{th}$ crossing in the $k^{th}$ orbit) 
where $N_k$ is the number of crossings in the $k^{th}$ orbit. To assess the periodicity of the crossing
intervals, we define the {\em aperiodicity} as
\begin{eqnarray}
a_k=\sigma_k/\overline{\Delta t_k}.
\end{eqnarray}
The lower the aperiodicity is the higher the periodicity is.
%%%%% I don't know if we should cancel the above sentence because it is
%%%%% obvious. 
In particular, an orbit with $a=0$ is strictly periodic.

We will investigate the variation of the aperiodicity of the solar orbit with the six parameters (initial conditions).
This is too large to report on exhaustively here, but we find that the aperiodicity is mostly sensitive to $R(t=0)$ and
$\dot\phi(t=0)$. This is because for the values listed in Table~\ref{tab:initialconditions}, they have the largest influence on the galactic potential experienced by the Sun. 
%%% not entirely clear, and perhaps also too much detail?
%In addition, therelative uncertainties of the crossing intervals and initial conditions are of the same order of magnitude. This means that the system has a translational symmetry of perturbation, i.e. the orbit is relatively stable with limited perturbation of initial conditions. 
In the following we vary these initial conditions individually, by drawing
$10^4$ samples from the corresponding initial condition distribution. In
Section~\ref{sec:sensitivity_biodiversity} we will find the final evidences for most models
are not sensitive to the sample size. 

\subsubsection{\label{sec:midplane_biodiversity} Midplane crossings}

Some previous studies have claimed that the Galactic midplane crossing triggers increases in terrestrial extinction due to an increased gamma ray or cosmic ray flux or perturbation of the Oort cloud. These are directly related to 
the increased stellar density and increased occurrence of star forming
regions. The increased tidal forces are postulated to enhance the disruption
of the Oort cloud \citep{rampino00, matese95}, and the higher density of massive stars -- and thus high energy radiation as well as increased supernova rate -- raise the average flux the Earth is exposed to.
%%% The following sentence is not quite clear: you need to make the point that this is an extragalactic mechanism.
%%% Please check that paper again.
%%%%% I have added something to make the sentense clearer
A related argument is that Galactic north--south anisotropy of CR production
and the CR propagation in galactic magnetic fields in the Galaxy modulated the CR flux on the Earth through the Sun's vertical oscillation \citep{medvedev07}.  The periodicity of the Sun's vertical motion -- not least its period, phase and the assumed stability of this period -- are central to these claims.  We examine these using our model.

\begin{figure*}
\centering
\includegraphics[scale=0.7]{sensitivity_planecross_itv.eps}
\caption{Periodicity test of midplane crossings varying just the current galactocentric radius of the Sun, $R(t=0)$.
 Top left: distribution of this initial condition in the simulations (it has a Gaussian distribution with parameters given in Table~\ref{tab:initialconditions}). Top right: cumulative probability of the aperiodicity parameter for the resulting orbits. Bottom left: the variation of aperiodicity with $R(t=0)$. Bottom right: the variation of aperiodicity with the average crossing interval, $\overline{\Delta t_k}$.}
\label{fig:sen-varyR-plane} 
\end{figure*}

The results of varying just the initial galactocentric radius of the Sun,
$R(t=0)$, are shown in Fig.~\ref{fig:sen-varyR-plane}. We see in the
top-right panel that about 90\% orbits have an aperiodicity less than 0.1. In the lower two panels we see how $a$ varies with the value of the initial condition and with the average crossing interval. 

The aperiodicity is 0.002 (nearly strict periodicity) at $\overline{\Delta t}=61.8$\,Myr.  
%%% Be more specific here: is this a 4:1 resonance (radial period to vertical period)?
%%% Is it also circular?
This corresponds to a 1:1 resonance between the vertical motion and the radial
motion. Its value is close to a period in the biodiversity data of $62\pm 3$\,Myr claimed by \cite{rohde05}. Not much should be read into this coincidence, however, as there is no good (i.e.\ independent) reason to select the specific initial condition that leads to this period over any other. 
Moreover, changing the parameters of the Galactic potential -- which is not very well known -- changes this period. 
%%% Please confirm that the following is true
%%%%% Yes!
For example, if we increase the mass of the Galactic halo the values of
$\overline{\Delta t}$ are decreased. The other minimum in the aperiodicity in
the bottom panels is 0.02 at $\overline{\Delta t}=100.2$\,Myr. This
corresponds to an approximately circular orbit in the midplane. If we set $V_R(t=0)=0$, $V_z(t=0)=0$ and $z=0$, this solar orbit would be strictly circular.

%%% The meaning of the following sentence is not clear. What do you mean by
%%% "one-to-four"?
%%%%% Here I just want to say the accumulative curve has a sharp turn because
%%%%% the number of values of R(t=0) corresponding to an apeirodicity changes
%%%%% from four to one after the turn. 
The accumulative curve has a sharp turn at $a'=0.1$ because the number of
values of $R(t=0)$ corresponding to each aperiodicity changes from four to one after the turn.
%%% You need to be clear about the cause of the following or else the reader may suspect you have done
%%% something wrong, or haven't bothered to find out what's going on
The discontinuity in the bottom graphs is caused by discontinuities in the
number of plane crossings achieved in an orbit. 

If we now vary the initial condition $\dot\phi(t=0)$ instead, the periodicity test gives very similar results: we find a nearly strict periodicity at $\overline{\Delta t}=60$\,Myr and another minimum in the aperiodicity at about 100\,Myr. That means the nearly strict periodicity is mainly determined by a combination of $R(t=0)$ and $\dot\phi(t=0)$.

In summary, we see that the majority of the simulated orbits (90\%) are quite close to periodic ($a\leq0.1$) in their motion vertical to the midplane, although strict periodicity essentially never occurs.
 
\subsubsection{\label{sec:spiral_biodiversity} Spiral arm crossings}

Regarding spiral arms as regions of increased star formation activity and stellar density, the mechanisms of mass extinction considered for midplane crossing could likewise be applied to spiral arm crossings, and have been by various authors \citep{leitch98, gies05}. However, such studies have over-simplified the solar motion by failing to take into account the considerable uncertainties in the current phase space coordinates of the Sun and thus in its plausible orbits.  Furthermore, some studies have even claimed a connection between spiral arm crossings and the terrestrial biosphere after having fit the solar motion to the geological data, a master stroke of circular argumentation.
%%%%%Rene comments on the last sentence that it is a little cynical. Maybe we
%%%%%should cancel the words after although. 

We examine here the periodicity of spiral arm crossings (although we note that some studies in the literature claiming a spiral arm-extinction link just consider the crossing times and do not claim a periodic crossing).
%%% Should this be two or three here? You referred to "at least two" and then to "more than two".
%%%%% "At least two" is the right one. In fact, if there were only two
%%%%% crossings, the interval should be zero, this could explain why there are
%%%%% some points with a=0 which does not mean the arm crossing is strictly
%%%%% periodic but only mean there is only one crossing. 
The crossing intervals are longer than with the midplane, so we only include
in our analyses models in which there are at least three arm crossings. We
assume that the arms have indefinite vertical extent, so that a crossing on the x--y plane is always a true encounter. In reality the Sun might pass over or under the arms, thus reducing the overall relevance of spiral arm crossings to terrestrial extinction.
%Different from midplane crossings, the solar orbit might miss the arm or tangent to the arm. We only kept simulations with more than two arm crossings because otherwise the standard deviation of intervals ($\sigma(\Delta t)$) would make no sense.

\begin{figure*}
\centering
\includegraphics[scale=0.7]{sensitivity_armcross_itv.eps}
\caption{As Fig.~\ref{fig:sen-varyR-plane}, but now for the spiral arm crossings.}
\label{fig:sen-varyR-arm} 
\end{figure*}

Fig.~\ref{fig:sen-varyR-arm} shows the result of this analysis for the 7\,407 orbits (out of the original sample of 10\,000) which exhibit at least three arm crossings.  The cumulative probability graph shows that about 40\% of the orbits have an aperiodicity larger than 0.2. In other words, it is not very likely that the solar orbit and spiral arms are so tuned to give highly periodic crossings.  The lower two graphs show how $a$ varies with $R(t=0)$ and $\overline{\Delta t_k}$.  The numerous gaps in these plots are simply a consequence of the fact that all orbits for certain ranges of $R(t=0)$ did not have at least three arm crossings, so were removed from the analysis. In other words, the crossing interval is very sensitive to $R(t=0)$.

In summary, we find that it is unlikely that spiral arm crossings are even close to periodic. If the pattern speed of the spiral arms has not been constant in the past 550\,Myr, or if the pattern itself has not been stable, then this conclusion is just strengthened further.

\subsection{\label{sec:OBM_biodiversity}Orbital model}

\subsubsection{Principle}

As outlined in Section~\ref{sec:introduction_biodiversity}, various astronomical mechanisms for biological extinction have been identified, including comet impacts (Oort cloud perturbation), gamma rays (SNe), and cosmic rays (SNe remnants) \citep{ellis95,sanchez01,gies05}.  The intensity of all of these depends on the local stellar density. More specifically, if we consider a mechanism involving flux from nearby stars -- such as gamma rays from a SN -- then the flux from a single star is proportional to $f/d^2$, where $f$ is the relevant surface flux from the star and $d$ is its distance. The sum of this over the whole relevant volume of space around the Sun is proportional to the total intensity and thus the extinction probability (per unit time). 

Let us assume that the extinction rate, $E$, is linearly proportional to the
SNe flux, and that the number density of SNe is proportional to the stellar
number density (stars per unit volume), $n$.  We shall further assume that
that the SN rate is constant in time and space and the intrinsic SN luminosity
is the same for all SNe.
In an axisymmetric cylindrical coordinate system, the extinction rate at the Sun is then
\begin{eqnarray}
E(R_\odot, z_\odot) &=& C \int \!\! \int \frac{n(R,z)}{d^2} \,R\,dR\,dz\nonumber\\
                           &=&C \int \!\! \int \frac{n(R,z)}{(R-R_\odot)^2+(z-z_\odot)^2}\,R\,dR\,dz,\nonumber\\
\label{eqn:stellar_density1}
\end{eqnarray}
where $R$ and $z$ are the galactocentric radius and height above the midplane, respectively, for a star,
$R_\odot$ and $z_\odot$ are the corresponding (time-varying) coordinates of the Sun,
and $C$ is a constant. If we define the distance from the SN to the Sun as $r\equiv R-R_\odot$ and $Z\equiv
z-z_\odot$, the extinction rate is  
\begin{eqnarray}
 E(R_\odot,z_\odot) &=& C \int \!\! \int\frac{n(R_\odot+r,z_\odot+Z)}{r^2+Z^2}(R_\odot+r) drdZ \ .\nonumber\\
\label{eqn:stellar_density2}
\end{eqnarray}
%%% Maybe we need to give a better justification of why we select 50pc
The flux from a SNe falls off as $1/d^2$, but we can anyway truncate this integral at some upper distance because
at some point the flux is too weak to influence the terrestrial biosphere. We
take $d_{\rm th}=50$\,pc as an upper limit.\footnote{\cite{ellis95} conclude that SNe which come within 10\,pc of the Sun
  would have a significant impact on terrestrial life.
GRBs up to 1\,kpc or even slightly more could still have an effect on the
Earth, but we ignore these because the GRB rate (at low redshifts) is just
about 11~Gpc$^{-3}$yr$^{-1}$ \citep{pelangeon08}. If we assume the number
density of typical galaxies to be $3\times 10^{-3}$~Mpc$^{-3}$ and the radius
of the Galaxy to be 15~kpc, this local GRB rate corresponds to an event rate within 1\,kpc of the Sun of just $6$\,Gyr$^{-1}$.}.
% $0.44$\,Mpc$^{-3}$Gyr$^{-1}$\citep{guetta05}, 
%%% Problem here:
%%% You originally had $0.44$\,Gpc$^{-3}$yr$^{-1}$, which is $0.44$\,Mpc$^{-3}$Gyr$^{-1}$
%%% which is $0.44e^{-9}$\,kpc$^{-3}$Gyr$^{-1}$, which is far lower than the number you give below,
%%% which is $7e^{-10}$\,yr$^{-1}$ or $0.7$\,Gyr$^{-1}$
%%% Or more directly: 1 per Gpc per yr = 10^-9 per kpc per Gyr
%%% So have you somehow integrated over the volume which the Sun passes through?
%%% It seems you anyway took the wrong number from Guetta et al. 2005. Just from the abstract I see
%%% "The inferred overall local GRB rate is $33\pm11 h_{65}^{3}$ Gpc$^{-3}$yr$^{-1}$."

This is much smaller than the scale length of the disk and comparable to the scale height of the disk (see Table~\ref{tab:model_par}), so we can approximate $n(R_\odot+r,z_\odot+Z)(R_\odot+r)\approx
n(R_\odot,z_\odot+Z)R_\odot$. The integral then becomes
\begin{equation}
E(R_\odot,z_\odot)\simeq CR_\odot\int_{-d_{\rm th}}^{d_{\rm th}}\int_{-d_{\rm th}}^{d_{\rm th}}\frac{n(R_\odot,z_\odot+Z)}{r^2+Z^2} drdZ \ .
\label{eqn:extinctionPDF1}
\end{equation}
Integrating over $r$ gives
%%% I think you forgot a factor of two here: please check. It doesn't actually matter because we're
%%% neglecting constants, but we don't (want to) change the constant C' again, so let's keep such factors.
\begin{equation}
E(R_\odot,z_\odot)\simeq 2CR_\odot\int_{-d_{\rm th}}^{d_{\rm th}}n(R_\odot,Z+z_\odot)\frac{\arctan(d_{\rm th}/Z)}{Z}\,dZ \ .
\label{eqn:stellar_density3}
\end{equation}
%%% If you plot $\frac{\arctan(d_{\rm th}/Z)}{Z}$ you'll see that it is still well above zero at 10-20pc, i.e. almost half
%%% of d_th, so it's a bit too extreme to characterize this as a delta function.
The geometric factor $\frac{\arctan(d_{\rm th}/Z)}{Z}$ drops close to zero at about $Z=$\,25\,pc, and does so much more rapidly than the stellar density term, which follows the vertical profile of the disk, which has a much larger scale height (250\,pc).
Thus to a reasonable degree of approximation we can set $n(R_\odot, Z+z_\odot)
\simeq n(R_\odot, z_\odot)$ in this integral. The integral is then just over
the geometric factor, which gives some constant (dependent on $d_{\rm th}$,
but of no further interest).
%\footnote{In the integration of geometric factor,
%  we avoid the domain with $r^2+Z^2\le 1$\,pc because the real stellar density in that
%  region should be zero.}.
%%% I assume the above is true, i.e. the integral does converge, even though 1/Z -> infinity. What, incidentally,
%%% is the result of the integral (in terms of d_th)?
Thus we are left with 
\begin{equation}
E(R_\odot,z_\odot)\simeq C'R_\odot n(R_\odot,z_\odot),
\label{eqn:stellar_density4}
\end{equation}
for some constant $C'$. For the solar motion, the relative
variation of $R_\odot$ is less than that of $n(R_\odot,z_\odot)$, so we have
\begin{equation}
E(R_\odot,z_\odot) \propto n(R_\odot,z_\odot) \ .
\label{eqn:stellar_density5}
\end{equation}
In other words, the extinction rate is just proportional to the stellar density at the location of the Sun. Hereafter, we will use the sum of the spiral density and the stellar density derived from the potential (see equation \ref{eqn:}) using Poisson's equation. 

%%% Presumably you derive n(R_\odot,z_\odot) from the equations for the potential using Poisson's equation?
%%% If so, mention this somewhere appropriate so that the readers know the potential and mass density are
%%% self-consistent. If not, how do you derive it?
In the above model we assumed that the extinction rate is proportional to
$d^{-2}$, i.e.\ the influence falls off like a flux on the surface of a
sphere. We could generalize this dependence to be $d^{-k/2}$ for $k\geq0$ in
order to reflect other mechanisms, e.g.\ tidal effects. 
%%% I don't think we need this
%For the model with $k\neq 0$, the extinction rate is still proportional to the stellar density at Sun's location given a small integration area because the distance factor varies intensively around Z=0. Note that the stellar number density can be a predictor of the extinction rate only when both $d_{\rm th}<<a_d$ and $d_{\rm th}<<b_d$.

In order to test the validity of the above approximations, we compare in Fig.~\ref{fig:ext-pos10}
extinction rate as given by equation~\ref{eqn:stellar_density1} (by numerical
integration) with the stellar number density $n(R_\odot, z_\odot)$. We show
the ranges of $R_\odot$ from 5\,kpc to 10\,kpc and $z_\odot$ from -0.5\,kpc to
0.5\,kpc, in accordance with the approximate range of the simulated solar orbits in Section~\ref{sec:periodicity_biodiversity}. 
As extinction rate is proportional to the computed quantities, we normalize by
setting the integral of the extinction rate over 
$R_\odot$ and $z_\odot$ to be one (and likewise for the stellar density).
\begin{figure*}
\centering
\psfrag{Rs}[c][c]{\scriptsize{$R_\odot$/kpc}}
\psfrag{Zs}[c][c]{\scriptsize{$z_\odot$/kpc}}
\includegraphics[scale=0.7]{ext-exact-pos10.eps}
\caption{Comparison of the extinction rate calculated numerically with the stellar density at the position of the Sun.
The top row shows the variation as a function of $z_\odot$ with $R_\odot$ fixed to 8\,kpc. The bottom row show the variation as a function of
$R_\odot$ with $z_\odot$ fixed to 26\,pc. The columns from left to right are for $k=0,2,4$ in the model for the dependence of extinction rate with distance.}
\label{fig:ext-pos10}
\end{figure*}
In the upper row of Fig.~\ref{fig:ext-pos10}, the difference between the stellar density and the extinction rate reaches a maximum in the midplane ($z_\odot=0$); this is on account of the relatively large density gradient at $z_\odot=0$. The maximum difference is only about 10\% of the peak value of stellar density for all values of $k$. In the lower row, the largest discrepancy between $n(R_\odot, z_\odot)$ and $E(R_\odot, z_\odot)$ is at the lower limit of $R_\odot$.
% "largely because the density gradient increases with the decrease of $R_\odot$."
%%% that is just is a description rather than an explanation. The issue is why does the extinction rate flatten off
%%% even though the density rises more steeply? The extinction rate includes the density, so the geometric factor
%%% must be acting strongly against this. If you can work it out, add a senetnce explaining that.
Note that the value of $k$ has very little impact.

In practice, most of the simulated orbits spend most of their time in the
region $7<R_\odot<9$ (\,kpc) and $-0.3<z_\odot<0.3$ (\,kpc), where the differences between local stellar density and extinction rate variation are even smaller. Thus to a few percent, the stellar density at the Sun is a good predictor of the extinction rate. The time variation of this is the time series model that we refer to as the ``orbital model'' (OM) in Section~\ref{sec:tsmodels_biodiversity}. 

$E(R_\odot,z_\odot)$ is the prediction of the extinction probability (per unit
time) from the orbital model: once normalized it is just the quantity $P(t |
\theta, M)$ in Section~\ref{sec:tsmodels_biodiversity}. The parameters of this model are the initial conditions, and the corresponding priors are Gaussian
distributions summarized in Table~\ref{tab:initialconditions}. Thus one orbit
calculated from one draw of the initial conditions allows us to calculate one
likelihood for this model (for given data set). Repeating this gives many
draws of the initial conditions and averaging (Section~\ref{sec:calcevi})
results in the evidence for the orbital model.

\subsubsection{Semi-orbital model}

%%% Are you totally sure than SOM is defined in this way and that it is not just an ADDITION of a constant to OM?
%%% If so, I suggest you read Feulner 2011 and decide whether you want to citep that here, as I think he proposes
%%% something similar. (I know it's not such a difficult idea as to need citing, but it's worth citing work which does
%%% something similar.)
We derive another model from the above orbital model. This ``semi-orbital model'' (SOM) 
assumes that there is a minimum level of background extinction, $h$, imposed
on to the variable extinction produced by the orbital motion (A similar model
could be found in \cite{feulner11}). The result is
a truncation of the orbital-induced extinction probability function to a
minimum level (see Fig.~\ref{fig:som}). We will investigate the SOM model
with h=0 in detail in Section~\ref{sec:result_biodiversity}. 
(Note that, as with all the models, this must be normalized so that the integral of $P(t | \theta, M$) over the time span of the data is unity.)
%%% I do not see why you have two paramters here: It seems to me that there is only one, and TH is determined from B.  I have assumed this is correct and replaced them with one, h. We do not need to define h exactly, as only the concept matters for the paper.
% For a simulated orbit, extinction rate is constant (i.e. background B) when stellar density is below the threshold (TH). When the stellar density is higher than TH, the extinction rate is proportional to the stellar density. Thus the SOM model is parameterized by initial conditions of the Sun, TH and B.

\begin{figure*}
\centering
\includegraphics[scale=0.7]{som.eps}
\caption{The orbital model (OM) and derived semi-orbital model (SOM). The left
  panel show the variation of the local stellar density -- and thus the
  extinction probability per unit time -- in one particular orbit calculated
  from OM. The horizontal dashed line is a threshold for truncating the stellar
  density, which then gives rise to the extinction probability per unit time
  plotted in the right panel with a background h (dotted line).}
\label{fig:som}
\end{figure*}

\section{\label{sec:result_biodiversity} Results}

\subsection{\label{sec:evidences_biodiversity} Evidences}

\begin{table*}
\caption{Bayes factors and maximum likelihood ratio of the various time series models (rows) relative to the uniform model for the various data sets (columns). OM1--4 refer to the OM model in which different initial conditions are varied: $R(t=0)$, $\phi\dot(t=0)$, $\{R(t=0),~\dot\phi(t=0)\}$, $\{R(t=0),~V_R(t=0),~\dot\phi(t=0),~V_z(t=0)\}$, respectively, and likewise for the SOM1--4 models. The other initial conditions are kept fixed.}
\centering
\begin{tabular}{l|llll|llll}
\hline
\hline
     &\multicolumn{4}{c|}{Bayes factor (BF)}&\multicolumn{4}{c}{Maximum
       likelihood ratio (MLR)}\\
\hline
Model&B5   &B18   &RM  &A08 &B5 &B18 &RM  &A08\\
\hline
PNB &0.97 &0.64   &0.98&0.87&22 &250 &1.2&1.1\\
PB  &1.0  &0.80   &0.98&0.87&3.5&45  &1.1&0.99\\
QPM &0.99 &0.85   &0.98&0.87&6.8&35  &1.1&0.98\\
RNB &0.041&0.00050&0.99&0.97&1153&16 &2.5&1.7\\
RB  &0.85 &0.40   &0.98&0.91&9.0&8.4 &1.4&1.2\\
SP  &0.28 &0.019  &1.02&0.88&2.7&0.36&2.1&1.3\\
SSP &0.73 &0.18   &0.99&0.87&8.6&81  &1.3&1.2\\
OM1 &1.3  &0.78   &0.99&0.91&4.0&2.7 &1.1&1.0\\
OM2 &1.3  &0.70   &0.99&0.92&4.4&2.4 &1.2&1.0\\
OM3 &1.3  &1.2    &0.99&0.87&4.0&2.8 &1.3&1.2\\
OM4 &1.2  &1.2    &0.99&0.87&5.1&2.8 &1.3&1.2\\
SOM1&0.86 &0.074  &1.0 &0.96&3.5&0.69&1.2&1.2\\
SOM2&0.78 &0.093  &1.0 &0.98&3.8&0.78&1.3&1.2\\
SOM3&0.88 &0.16   &0.99&0.88&3.5&0.82&1.4&1.3\\
SOM4&0.74 &0.16   &0.99&0.88&8.9&0.82&1.4&1.3\\
\hline
\end{tabular}
\label{tab:BF-MLR}
\end{table*}

We now calculate the Bayesian evidence (equation~\ref{eqn:evidence}) for the
various models for the various data sets. This is done by sampling from prior
probability distributions of the model parameters ($P(\theta | M$),
Table~\ref{tab:prior}), calculating the likelihood
(equation~\ref{eqn:likelihood_disc} for discrete time series,
equation~\ref{eqn:likelihood_cont} for continuous time series) and then
averaging these for that model and data set (\ref{eqn:evidencenum}). 

%%%%% Rene has commented that the 10^4 sample might not large enough to reduce
%%%%% the statistical uncertainties propagated into the BF. Shall we test the
%%%%% sensitivity of the evidence to the sample size? In fact, I have already
%%%%% changed the sample size for some models. I think only the random model
%%%%% without background is sensitive to the sample size. For other models
%%%%% especially the ones with background, the sample size is not important. 
For RNB and PNB models for the B5 and B18 data sets, we adopt a Monte Carlo
sample size of $10^6$. In all other cases we use a sample size of
$10^4$. This choice of sample size is according to the sensitivity test of the
evidence to the sample size for all models and all data sets. This test shows
that the evidence estimated from $10^4$ draws in the prior distribution is
close to the real evidence when there is a background either in the model or
in the data set. Thus, considering the computing time, we only calculate the
evidence for the RNB and PNB models for the B5 and B18 data sets with a sample
of $10^6$.
%%%%%%The following graph is actually for the section of sensitivity
%%%%%%test. However, because the sample size is neither a real parameter of model nor an observable of the data, so I just mention the result in above paragraph.
%The numerical calculation of evidence for a model is only an estimation of the
%true evidence. Thus the evidence may be sensitive to the sample
%size.
%To test the sensitivity of the evidences for the obital model, we repeat the
%numerical calculation of the evidences for OM1 and SOM1 for the B18 data
%set. Each evidence is calculated from a sample of 10,000 initial condition
%sets, and the calculation is repeated 10 times. We find that the relative
%change of the evidence is less than 5\% for both models. We also test the
%sensitivity of the evidence for other time series models for the B18 data set
%with the this method. We find that the evidences for other models with
%background or trend are not sensitive to the sample size (with a factor less
%than 2\%). However, the evidences for the models without background, i.e. RNB
%and PNB, are sensitive to the sample size. In addition, the sensitivity test
%for other data sets shows that the evidence estimated from 10,000 draws is
%close to the real evidence when there is a background either in the model or in the data set. Thus, for the RNB and PNB models, we calculate the corresponding
%evidences from a sample of $10^6$ points. For other models, we use a sample
%size of 10,000. 

The Bayes factor (BF) is the ratio of two evidences. Here we form Bayes
factors with respect to the uniform model. We may regard a model as
significantly better than another when its evidence exceeds that of the other
by a factor of ten \citep{jeffreys61, kass95}. Note that it is only meaningful to compare evidences -- and therefore Bayes factors -- for a fixed data set.

The results are shown in Table~\ref{tab:BF-MLR}. For the reference models we evaluate the evidence by sampling over all their model parameters, but in the case of OM and SOM we sample over just some of the parameters (initial conditions), keeping the others fixed, in order to investigate the impact of the different parameters.  As shown in Section~\ref{sec:periodicity_biodiversity}, the periodicity of solar orbit is most sensitive to the initial conditions $R(t=0)$ and $\dot\phi(t=0)$. We therefore calculate the evidence for the OM (and SOM) models with four different sets of initial conditions being varied: $R(t=0)$ only; $\phi\dot(t=0)$ only; $\{R(t=0)$ and $\dot\phi(t=0)\}$; $\{R(t=0)$, $V_R(t=0)$, $\dot\phi(t=0)$, and $V_z(t=0)\}$.  In all cases we fix $\phi(t=0)$ and $z(t=0)$, the former because it has no impact on the solar motion in this axisymmetric potential, and the latter because the uncertainty in the current $z$ position of the Sun has a limited impact on the subsequent orbit.

For the B5 data set, the BFs of all time series models relative to the uniform model are less than 10. This means that we have no evidence for identifying any of these models as a better explanation of the data. Given that the uniform model is the simplest model of the set, the principle of parsimony leads us to be satisfied with it as explanation. This of course does not deny the possibility that an untested model could show significantly higher evidence. After all, we can only ever make claims about models which we explicitly test.\footnote{It is worth noting that classical hypothesis testing, e.g.\ using p-values, never explicitly tests the model of interest, the so-called alternative hypothesis. It works instead by ``rejecting'' some null hypothesis. This is then interpreted as acceptance of the alternative hypothesis. However, this only follows if the two hypotheses cover all possibilities -- one is the complement of the other -- which is rarely the case. Bayesian model comparison, in contrast, treats all models.} One model, RNB, has a Bayes factor less than 0.1, indicating that we can discount this one as being an unlikely explanation.

The B18 data set includes more extinction events than the B5 data set, and not surprisingly we see that this data set discriminates more strongly between the time series models (the Bayes factors show a larger spread). The OM models are favoured somewhat more than the other models -- e.g.\ the BF of OM3 to SP is $1.2/0.019=63$ -- although again no model is favoured significantly more than the uniform model. In contrast, several models are significantly disfavored (RNB, SP, SOM1, SOM2).  These results are shown graphically in the left panel of Fig.~\ref{fig:BF-MLR}.

\begin{figure}
\centering
\includegraphics[scale=0.7]{bar_evi_comp_B18.eps}
\includegraphics[scale=0.7]{bar_like_comp_B18.eps}
\caption{Results for the B18 data sets. The left panel shows the log (base 10)
  Bayes factor of the various models relative to the Uniform model. The right panel shows the log (base 10) of the maximum likelihood ratio of various models relative to the Uniform model.
} 
\label{fig:BF-MLR}
\end{figure}

For the two continuous time series, RM and A08, the difference between the
evidences of all of the models is not significant. We also find that the evidence for SOM is not sensitive to $h$.
% We have varied TH and B and find that the evidence for the SOM model for continuous data is not sensitive to these two parameters. 

Our broad conclusion is that no model significantly outperforms the uniform model on any of the data sets. On the contrary, a few can be ``rejected'' on the ground of a significantly lower evidence. Recall that all of these models are predicting the extinction probability (per unit time). In terms of the discrete data sets, the uniform model just means that the mass extinction events occur at random in time. We find this to be no less probable than a periodic or quasi-periodic variation of the probability, or a monotonic trend in the probability, etc.  In terms of the continuous data sets, we clearly do not believe that the uniform model is a good explanation of the clearly apparent variations in the extinction rate (see Fig.~\ref{fig:data}). But the analysis does tell us that this is no worse an explanation than more complex models of the variation, such as periodic, orbital-model based etc. Clearly there must be yet other models which could explain the data even better.  This may explain why previous authors have found an apparent periodicity in the data: the periodic model can explain the data to some degree, but actually no better than simpler models.


\subsection{\label{sec:likelihood_biodiversity}Likelihood distribution}

We have seen that the evidence provides hardly any discrimination between any of the models on the continuous data, nor for many of the models on the discrete data sets.  (This is by no means inevitable. In other problems the evidence can vary enormously between models.)  This means that, on average over their parameter space, the models differ little in their predictions. As the evidence is just the average of likelihood samples, we can simply plot these samples to investigate how the likelihood varies with the parameters. We focus here mainly on the PNB, OM and SOM models for the B18 data 

%%% CHANGE axis label on right panel to be "log likelihood ratio"
%%%%% However, here we cannot define the likelihood ratio of the PNB and
%%%%% Uniform model as Bayes factor
\begin{figure}
\centering
\includegraphics[scale=0.7]{like_periodic_B18_2D.eps}
\includegraphics[scale=0.7]{like_B18_periodogram.eps}
\caption{Likelihood distribution for the PNB model on the B18 data set as a function
of period and phase (left panel) and period only (right panel).
In both panels we show the
likelihood ratio of the PNB to the Uniform model, on the left as log (base 10) 
on a color scale.}
\label{fig:like-2D-pnb}
\end{figure}

Fig.~\ref{fig:like-2D-pnb} shows how the likelihood varies over the
two-dimensional space formed by the two parameters, period and phase, of the
PNB model. There is significant variation. We see numerous local maxima, the
largest likelihoods being around $\{T/Myr,~\beta/rad\}=\{60,
4.5\}$.  However, these maxima are rather narrow, so once the likelihood in
the other (equally plausible) regions are taken into account, the overall
evidence for the model is not particularly high.  If we are interested in the
variation of likelihood with just the period, then we can marginalize this
diagram over phase, and plot with respect to period, thereby forming a
(Bayesian) periodogram (right-hand panel). We see a clear peak around 60\,Myr. This is
coincident with the period of $62\pm 3$\,Myr identified by \cite{rohde05}. It is tempting to associate this peak value of the
likelihood with the periodic model as a whole, and use it to claim a larger
evidence for the periodic model. Certainly there is a degree of arbitrariness in
the prior parameter distribution -- in this case a uniform distribution -- and
narrowing this range around this peak would clearly increase the evidence.
For example, if we truncate the period range from its current value of
[10,\,100]\,Myr to [50,\,80]\,Myr, then the Bayes factor relative to the
uniform model increases from 0.64 to 1.5. This is a rather modest increase, but we could increase it to a significantly high value with an even  narrower prior. However, we should not use the data to find the best fitting parameters and then claim that we should only consider the model over this range! We would need some other reasoning or independent data for making such a selection. (The \cite{rohde05} time series is not independent from B18, as they are both based on the same paleontological data.) We do not see how, a priori, we could limit the plausible periods of periodicity to something as narrow as 50--80\,Myr, let alone the much narrower range required to favour PNB significantly over other models. In the extreme limit of an infinitesimal region around the maximum likelihood, we end up doing model comparison using the maximum likelihood. Just out of interest, these values are shown in Table~\ref{tab:BF-MLR} and plotted in Fig.~\ref{fig:BF-MLR}. If we were to use this (incorrect) metric, then PNB and some of its variants have significantly higher evidence than the uniform model and several of the other models (although barely more than a factor of ten above the random model, RB). Another way of seeing why this is the wrong approach was already discussed in Section~\ref{sec:overview}: by focusing on the {\em best} fits, we simply favour the more complex model. We could always define a more flexible model and so fit even better.

We labor this point because many of the claims for a periodicity in biodiversity data have made use of a maximum likelihood approach (of which $\chi^2$ is a special case) or something equivalent.  We must instead use the evidence for model comparison. (Maximum likelihood may be used for estimating the best parameters once we've established we have the best model.) If the periodic model were in fact the true one, then of course only one period and phase would be true. In that case the likelihood around these values would be so high as to result in a large evidence even when averaging over the broader parameter space (see simulations in Section~4.1 of \cite{bailer-jones11} for a demonstration).

Incidentally, the fact that we find a dominant period at all in the B18 data set is actually not that unlikely. The (Bayesian) periodogram of samples drawn at random from a uniform distribution often exhibits a period 
which has a likelihood larger than that of the true uniform model (see Section~4.2 of \cite{bailer-jones11}). In other words, it is often possible to explain a random data set with {\em some} period, which is just a testament to how flexible the periodic model is.

%%% It would be better to show the bayes factor instead in the right-hand panels, which I think just means
%%% subtracting log10(4.06\times 10^{-50}) = - 49.59
\begin{figure*}
\centering
\includegraphics[scale=0.7]{likelihood_varyR_B18.eps}
\includegraphics[scale=0.7]{likelihood_varyphidot_B18.eps}
\caption{The variation of initial conditions (left column) and corresponding
  variation of likelihood ratio relative to the uniform model (right column) for the OM model on the B18 data set. The top row is for OM1,
in which only $R(t=0)$ is varied. The bottom row is for OM2, in which only $\dot\phi(t=0)$ is varied.}
\label{fig:like-r-phidot-B18}
\end{figure*}

Moving on from the periodic model, we show in Fig.~\ref{fig:like-r-phidot-B18}
the likelihood distribution for OM1 and OM2, i.e.\ where we vary the 
initial conditions $R(t=0)$ and $\dot\phi(t=0)$. 
As this shows likelihood on a log scale, the variations are a factor of $10^3$ to $10^4$.
%%% You had the following, which is not really true, because we have a log scale
In Fig.~\ref{fig:like-r-phidot-B18}, most part of the parameter space is favored
by the data on the same level with the uniform model, which reduces the
difference between maximum likelihood and the evidence. 
If we had lower uncertainties on these phase space coordinates of the Sun, then we could conclude something more definitive. For example, if $R(t=0)=7.5$\,kpc then the OM would be even less favored.
%%% Is the following therefore still true?
%%%%% Yes, I have changed the scale of likelihood distribution, the result for
%%%%% other models should be the same. 
We see a similar degree of variability for the other OM models and data sets listed in Table~\ref{tab:BF-MLR}.

We have likewise analyzed the likelihood distributions for the other models and data sets, but report only the maximum likelihood ratios (MLRs) in Table~\ref{tab:BF-MLR}. 

For the B5 data set, the RNB model has the highest MLR, yet its evidence was
the lowest. This indicates that while one particular instance of RNB fit the data well, overall it is a poor model.

For the RM and A08 data sets, the 
evidences are very similar for all models. This means that the data are not able to discriminate between these models very well, i.e.\ they are equally good (or bad).
However, the time series analysis model used here is not best suited to these data sets, as they can be better interpreted as valued time series, i.e.\ ones in which we have an extinction magnitude attached to each time (both, in general, with uncertainties), rather than a time variable probability of extinction.
%%% please add this to the bibliography
\cite{bailer-jones12} has extended the present model in order to work with such data sets; the results of its application to RM and A08 will be reported in a future publication.

In summary, we find that for none of the data sets is any model particularly favored beyond the simple uniform one.
In particular, there is no evidence to suggest that the orbital model (with or without a background extinction level)
is a particularly good explanation of the data.


\subsection{\label{sec:sensitivity_biodiversity} Sensitivity test}

The evidence is of course sensitive to the choice of prior
parameter distribution, and often we have little reason to chose a specific distribution. Here we test the sensitivity of the evidence to these, as well as to the parameters of the Galactic potential used in the orbital models, and to the age uncertainties for the discrete data sets.

%%% This plot is confusing. According to later text, you are including the results of the second 
%%% sensitivity test (varying N and B for the RB model) here also. If so, remove those results.
%%% 1. Your naming scheme 4sig vs sd4 is confusing. Why somestimes sig and sometimes sd?
%%% I suggest to use instead "Xsd", where X is the factor by which the sd has been changed,
%%% i.e. (1/4)sd, (1/2)sd, 2sd, 4sd. 
%%% The horizontal axis identifies the model, (S)OM1-4, so this does not need to appear in the name
%%% 2. The y-axis should be the Bayes factor (relative to the uniform model again).  Just label it "Bayes factor".
%%% This axis should not be the evidence for some model on one data set relative to another, as the definition of Bayes
%%% factor requires that the data be unchanged.
%%% ==>> Actually, because of this fact, we should be looking at the Bayes factors across models for a given data
%%% set. Therefore, please plot the figure such that the x-axis represents the four data sets (1/4)sd, (1/2)sd, 2sd, 4sd.
%%% Then using different plotting symbols to reflect the four models OM1-4 at each x value. In order to
%%% better separate OM from SOM, plot the four values for OM a distance dx to the left of the corresponding value of
%%% x, and the four values for OM the same distance to the right, with dx = 10% (or so) of
%%% the spacing between the marks on the x-axis. Thus at each x value (data set) we have two columns of points,
%%% one for OM the other for SOM.
%%%%% Here, I have included one more graph because I have not changed both the
%%%%% age uncertainties of the B18 data set and the uncertainties of the
%%%%% initial conditions simultaneously. Thus, I include two graphs with
%%%%% different varied uncertainty for each. 
\begin{figure}
\centering
\includegraphics[scale=0.7]{evi_comp_sig.eps}
\includegraphics[scale=0.7]{evi_comp_sd.eps}
\caption{The Bayes factor of the varied OM/SOM models (relative to the Uniform
  model) for the B18 data sets. In the left panel, the labels of the x axis (Xsd) denote the
  varied B18 data sets, where Xsd means multiplying the age uncertainties of the B18 time series by X (X=1/4, 1/2, 1, 2, 4). There are two columns of points
  corresponding to a data set: one for OM and the other for SOM. In the right
  panel, the labels of the x axis (Xsd) denote the varied uncertainties of the
initial conditions, where Xsd means multiplying the uncertainties of the
initial conditions by a factor of X (X=1/4, 1/2, 1, 2, 4). } 
\label{fig:priortest}
\end{figure}

The age uncertainties -- the expected noise in the data -- are taken into account by the likelihood function. However, it is often difficult to estimate uncertainties, and we further made a plausible, but not unique, translation of the estimated duration of a stratigraphic substage into age uncertainty (Section~\ref{sec:datadiscrete_biodiversity}). We therefore recalculate the likelihoods and evidences by scaling the standard deviation of the Gaussian representing each event by a constant factor. We do this for values of this factor of $1/4$, $1/2$, $2$, and $4$. 
For each of these data sets we calculate the evidences for the models (S)OM1--4 and the uniform model and recalculate the Bayes factors relative to the uniform model. 
%%% See notes on above plot to see what to plot.
%%%%%% Here, I include an additional description or conclusion based on the
%%%%%% additional graph. 
These are plotted in the left panel of Fig.~\ref{fig:priortest} for the B18
data set. We see that these changes in age uncertainties vary the Bayes
factors by factors of a few percent at the most. We also change the uncertainties of the initial conditions of the
orbital models. As a result, the changes of Bayes factors are insignificant either. Thus we conclude that our evidence results are robust to changes
in the age uncertainties (and to ambiguities in the definition of these) and
the uncertainties of the Sun's initial conditions. We see the same results for the B5 data set.
%%% How did you manage to conclude the following? The changes are no more than a factor of a few, which is not
%%% that much (and much less than the factor of 1000 variation in likelihood we saw for the parameters of the
%%% OM we had above, which you referred to as small (!).
%First, we vary the age uncertainties of the discrete data sets. We find that the evidence for RNB model is very sensitive to the age uncertainties of the discrete data sets. However, the RNB is never favored by the discrete data set better than the uniform model. In figure \ref{fig:priortest}, from the scale of log BF, we can find that the evidences for the OM/SOM models for the B18 data set is not sensitivity age uncertainties. It is the same case for other time series models and the B5 data set. 

%%% Do not plot these results in figure~\ref{fig:priortest}.
%%%%% I have added and changed some words for including the sensitivity test by changing
%%%%% the uncertainties in the simulated events
As a second sensitivity test, we allow the number of simulated random events,
$N$, and the age uncertainty of each event, $\sigma$, in the RNB and RB models to vary. Originally we fixed
$N=5$ when drawing models for the B5 data set and $N=18$ for the B18 data
set. For the B18 data set, we find that the more peaks the RNB model includes
and the bigger the uncertainty is the higher the corresponding BF is. However,
the RB model is not as sensitive to N and $\sigma$ as the RNB model (ref. Table~\ref{tab:sen-prior}). 
%%% The following is unclear. I think we don't need it once we've changed figure~\ref{fig:priortest}.
%%% Instead just report in words on the size of the changes we see.
%We find that the evidences for new models and the original model are of the same order of magnitude. We have also changed the standard deviation of the Sun's initial conditions. In figure~\ref{fig:priortest}, the variation of the evidence is still less than ten, which means the evidences for OM/SOM models for the B18 data set are not sensitive to the uncertainties of Sun's initial conditions.

%%% Report some more sensitivity tests to the parameter priors, i.e. the parameter ranges. 
%%% You could have a table in which you adopt half or quarter of the parameter range of each parameter
%%% for each model. E.g. if a parameter has range -1 to 1, then calculate the evidence for
%%% -1 to 0, 0 to 1, -0.5 to +0.5, and -0.25 to +0.25. That's just an idea. Experiment!
%%% You could do this for PNB, PB, QPM, SP, SSP
For the other models -- PNB, PB, QPM, SP, SSP -- we recalculate the evidence
using a different (narrower or broader) range of the prior. The Bayes factors
for other models with different priors are listed in Table~\ref{tab:sen-prior}.
We can see from the table that the BFs for PNB, PB, QPM, SP and SSP are not
sensitive to the range of the prior (the change is no more than a factor of 10).
\begin{table}
\caption{The BFs for time series models for the B18 data set with varied
  prior. The varied priors are listed in the second column, and for each
  varied prior, other priors are fixed. }%%%%%need to be checked
\centering
\begin{tabular}{l|c|r}
\hline
\hline
models&varied prior&BF\\
\hline
\multirow{4}{*}{PNB}
&none&0.64\\
&$50<T<80$&1.5\\
&$10<T<200$&0.31\\
&$10<T<400$&0.15\\
\hline
\multirow{3}{*}{PB}
&none&0.80\\
&$B=1/2$&0.88\\
&$B=2$&0.97\\\hline
\multirow{4}{*}{QPM}
&none&0.85\\
&$0<A_Q<1/4$&0.62\\
&$0<A_Q<1$&0.54\\
&$100<T_Q<300$&0.61\\
&$100<T_Q<500$&0.58\\\hline
\multirow{5}{*}{RNB}
&none&0.00050\\
&$\sigma=5$~Myr&$1.8\times 10^{-11}$ \\
&$\sigma=20$~Myr&0.026\\
&$N=9$&0.0085\\
&$N=36$&0.050\\\hline
\multirow{5}{*}{RB}
&none&0.40\\
&$\sigma=5$~Myr&0.73\\
&$\sigma=20$~Myr&0.25\\
&$B=\frac{1}{2\sqrt{2\pi}\sigma}$&0.13\\
&$B=\frac{2}{\sqrt{2\pi}\sigma}$&0.45\\
&N=9&0.84\\
&N=36&0.20\\
\hline
\multirow{4}{*}{SP}
&none&0.019\\
&$-200<\lambda<0$&0.070\\
&$0<\lambda<200$&0.10\\
&$10<t_0<500$&0.047\\\hline
\multirow{3}{*}{SSP}
&none&0.18\\
&$10<T<200$&0.17\\
&$-200<\lambda<200$&0.37\\
&$10<t_0<500$&0.27\\
\hline
\end{tabular}
\label{tab:sen-prior}
\end{table}

Finally, we test the sensitivity to the parameters of the potential in the
Galaxy model (ref. Table~\ref{tab:sen-model-par}). If we double the mass of the
halo, we find that the evidence for OM and SOM models for the B18 data set are
essentially unchanged. We also randomly draw 100,000 $M_h$ from a
Gaussian distribution with standard deviation of $M_h$ and vary $R(t=0)$ as
well. The final BFs for OM1 ans SOM1 are 0.69 and 0.14, which are comparable
with the ones listed in Table~\ref{tab:BF-MLR}. The Bayes factors of the (S)OM
models change by no more than a factor of 2 compared with the original (S)OM
models (see Table~\ref{tab:BF-MLR}). For all the changes of Galaxy parameters,
the varied BFs are either lower or no more than 3 times higher than the
corresponding original BFs. In addition, we can also add the perturbation of
spiral arms in the potential in the simulation of solar orbits. The change of
BFs for orbital models are limited. For example, for the OM1 and SOM1 models,
the difference between the BFs calculated from the perturbed orbits and the
ones listed in Table~\ref{tab:BF-MLR} is less than a factor of 10\%. 
%%%%% The above description need to be checked.
%%%%% I have also added the last two sentences to address the effect of the
%%%%% perturbation from spiral arm. The result show that the result is
%%%%% unsensitive to the perturbation.   
%%% Quantify the above, e.g. "(by no more than X%)".
%%% Report some more results here, e.g. changing the other parameters. This is quite
%%% important, as possible many people would think that changing the Galaxy parameters
%%% has a big impact.
\begin{table*}
\caption{The BFs for orbital models with different Galaxy parameters}
\centering
\begin{tabular}{l*{8}{c}}
\hline
\hline
orbital models  &OM1 &OM2 &OM3 &OM4 &SOM1 &SOM2 &SOM3 &SOM4\\
\hline
$none$   &0.78&0.70&1.2 &1.2 &0.074&0.093&0.16 &0.16\\
$2M_b$   &0.61&0.49&0.55&0.56&0.049&0.008&0.03 &0.031\\
$1/2M_b$ &0.79&0.88&0.66&0.67&0.064&0.093&0.052&0.051\\
$2b_b$   &0.79&0.79&0.67&0.67&0.080&0.078&0.054&0.055\\
$1/2b_b$ &0.78&0.80&0.67&0.66&0.071&0.068&0.050&0.049\\
$2 M_h$   &0.66&0.78&0.61&0.62&0.11 &0.116&0.093&0.097\\
$1/2 M_h$ &0.71&0.61&0.58&0.58&0.14 &0.045&0.11&0.11\\
$2 b_h$   &0.71&0.47&0.57&0.57&0.22 &0.043&0.17&0.17\\
$1/2 b_h$ &0.073&0.055&0.14&0.18&0.0039&0.002&0.017&0.022\\
$2 M_d$   &0.21&0.063&0.42&0.39&0.0033&0.004&0.044&0.040\\
$1/2 M_d$ &0.46&0.42&0.38&0.39&0.015&0.006&0.013&0.012\\
$2 a_d$   &0.91&0.95&0.80&0.80&0.12 &0.13 &0.088&0.090\\
$1/2 a_d$ &0.56&0.62&0.48&0.49&0.024&0.033&0.028&0.028\\
$2 b_d$   &1.2 &1.2 &0.95&0.93&0.033&0.058&0.034&0.33\\
$1/2 b_d$ &0.74&0.89&0.62&0.63&0.25 &0.35 &0.21 &0.21\\
\hline
\end{tabular}
\label{tab:sen-model-par}
\end{table*}

In summary, we find that the results are not particularly sensitive to the age
uncertainties, Galaxy model parameters, or reasonable changes to the prior
parameter distributions. (Of course, if we adopted a prior focused on a very narrow part of the parameter space, then we could get a much higher or lower evidence, but it would be unreasonable to adopt such a contrived prior.)


\section{\label{sec:conclusion_biodiversity} Summary and conclusions}

We have used a Bayesian model comparison method to calculate how well different time series models
can explain paleontological data sets recording the variation of biodiversity
over the Phanerezoic eon (the past 550\,Myr). One of these models is derived
from the orbit of the Sun around the Galaxy over this period, which has been
reconstructed from a model of the Galactic mass distribution. Our model
comparison takes into account uncertainties in the data as well as
uncertainties in the reconstructed path of the Sun. We have compared the evidence for this model with that of various other parametric reference models of no particular causal origin. All models are stochastic in the sense that they predict only the time variation of the extinction probability, rather than trying to predict the exact magnitude of the extinction rate or the times of mass extinctions.

As part of this analysis we investigated the properties of plausible solar orbits (i.e.\ those consistent with the limited accuracy of the present phase space coordinates of the Sun). We find that the majority of orbits have a motion perpendicular to the Galactic plane which are not far from periodic, although a precise period cannot be inferred due to the uncertainties in the present solar phase space coordinates as well as the exact mass distribution (gravitational potential) of the Galaxy. Thus any claims which try to link a variation in geological biodiversity, cratering or climate records to this solar motion must consider that motion to be quasi-periodic rather than strictly periodic.

In contrast, only about half of the simulated orbits showed periodic spiral arm crossings. Indeed, many of the orbits
did not encounter the spiral arms more than once. This conclusion is of course heavily dependent on the 
assumed model for the spiral arms and their pattern speed, both of which are
poorly known, and this fact alone means that any claims of a causal connection
between spiral arms and terrestrial conditions should be taken with a pinch of
salt.
 
We have shown how the evidence should be used to do fair model comparison, as opposed to selecting the model which gives the best single fit. The reason is that an arbitrarily complex model can always be tuned to fit the data arbitrarily well, yet that does not make it a good model.  By averaging the likelihood over the parameter space, the evidence uses the rule of probability to trade off the quality of the fit with the model plausibility in a quantitative fashion. Of the models investigated, we do not claim any one of them to be ``true''. Indeed, no model is exactly true in reality.  All we can hope to do is to find the best of the ones tested so far.

We find that none of the models tested explain the discrete data better than a uniform model. In other words, the time distribution of mass extinction events is consistent with being randomly distributed in time. There is no need to resort to anything more exotic.  

The uniform model is also no worse than other models for the continuous data sets. This does not mean that we believe the extinction rate has been constant over the Phanerezoic, but rather that none of the other more complex models is {\em significantly} better. Assuming the variations in extinction seen in Fig.~\ref{fig:data} are true -- which is well established -- then this tells us that there must be other models, not yet tested, which could explain the data better. This is investigated in a forthcoming publication using a model more suited for these types of time series.

We therefore find that the orbital-based extinction model is not favored by
the data. Recall that this model adopted an extinction mechanism in which the
extinction rate was proportional to the integrated ``flux'' (of a
non-specified type) from nearby stars, which was found just to be proportional to the stellar density local to the Sun.  This model was not favored partly because of the uncertainty in the exact orbit of the Sun, but perhaps also because this flux/density assumption is not correct. It does not necessarily mean that the solar motion plays no part in terrestrial extinction, nor that astronomical mechanisms are irrelevant.

Of course, it is quite plausible that the biological extinction rate has been affected by many factors, and so any attempt to connect them solely to the solar motion, or indeed to any simple analytic model, is doomed from the start. We have addressed this to some extent by including compound models and the semi-orbital model, but clearly one could be much more thorough. However, given the present uncertainties of the reconstructed solar orbit, it seems unlikely that one could draw a strong conclusion on the positive relevance of the solar orbit.  This, indeed, is the main conclusion of this work, plus the confirmation that periodic models are not a good (or necessary) explanation of the biodiversity variation.
%%% Add one or two recent references to Gaia
There is some hope that, in the future, results from the Gaia survey of the
Galaxy will improve our knowledge of the Sun's current location and velocity,
Galactic potential, spiral arms and inferred solar orbit to the extent that
this study can be repeated to give conclusions of greater certainty \citep{lindegren08,koposov09}.


==> zusammenfassung.tex <==

% This file contains the German version of your abstract, with about 300-500 words


